Chemical Reaction Network Decomposition Technique for Stability Analysis

This paper develops the concept of decomposition for chemical reaction networks, based on which a network decomposition technique is proposed to capture the stability of large-scale networks characterized by a high number of species, high dimension, high deficiency, and/or non-weakly reversible structure. We present some sufficient conditions to capture the stability of a network (may possess any dimension, any deficiency, and/or any topological structure) when it can be decomposed into a complex balanced subnetwork and a few 1-dimensional subnetworks (and/or a few two-species subnetworks), especially in the case when there are shared species in different subnetworks. The results cover encouraging applications on autocatalytic networks with some frequently-encountered biochemical reactions examples of interest, such as the autophosphorylation of PAK1 and Aurora B kinase, autocatalytic cycles originating from metabolism, etc.

==> decomposing CRN_SIADS (1)/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{CRN Decomposition for stability}{Y. Lu, C. Gao and D. Dochain}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Chemical Reaction Network Decomposition Technique for Stability Analysis\thanks{Submitted to the editors. \date{\today}.
\funding{This work was funded by the National Nature Science Foundation of China under Grant
No. 12071428, 11671418, and the Zhejiang Provincial Natural Science Foundation of China under Grant No. LZ20A010002.
}}}

% Authors: full names plus addresses.
\author{Yafei Lu\thanks{School of Mathematical Sciences, Zhejiang University (\email{11535029@zju.edu.cn (Y. Lu), gaochou@zju.edu.cn (C. Gao, Correspondence)).}}
\and Chuanhou Gao\footnotemark[2]
\and Denis Dochain\thanks{ICTEAM, UCLouvain, B\^{a}timent Euler, avenue Georges Lema\^{i}tre 4-6, 1348 Louvain-la-Neuve, Belgium (\email{denis.dochain@uclouvain.be (D. Dochain).}}}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

